Attacking Delay-based PUFs with Minimal Adversary Model

Physically Unclonable Functions (PUFs) provide a streamlined solution for lightweight device authentication. Delay-based Arbiter PUFs, with their ease of implementation and vast challenge space, have received significant attention; however, they are not immune to modelling attacks that exploit correlations between their inputs and outputs. Research is therefore polarized between developing modelling-resistant PUFs and devising machine learning attacks against them. This dichotomy often results in exaggerated concerns and overconfidence in PUF security, primarily because there lacks a universal tool to gauge a PUF's security. In many scenarios, attacks require additional information, such as PUF type or configuration parameters. Alarmingly, new PUFs are often branded `secure' if they lack a specific attack model upon introduction. To impartially assess the security of delay-based PUFs, we present a generic framework featuring a Mixture-of-PUF-Experts (MoPE) structure for mounting attacks on various PUFs with minimal adversarial knowledge, which provides a way to compare their performance fairly and impartially. We demonstrate the capability of our model to attack different PUF types, including the first successful attack on Heterogeneous Feed-Forward PUFs using only a reasonable amount of challenges and responses. We propose an extension version of our model, a Multi-gate Mixture-of-PUF-Experts (MMoPE) structure, facilitating multi-task learning across diverse PUFs to recognise commonalities across PUF designs. This allows a streamlining of training periods for attacking multiple PUFs simultaneously. We conclude by showcasing the potent performance of MoPE and MMoPE across a spectrum of PUF types, employing simulated, real-world unbiased, and biased data sets for analysis.

==> sections/Experiments.tex <==
\section{Experimental Results and Analysis}
\label{sec:exp}
\subsection{Data Preparation}
 We conduct experiments on three unique datasets: one simulated data built by an additive-delay model, one collected from PUF designs synthesised in hardware, provided by Mursi et al \cite{Mursi}, and the other biased data collected from a non-layout-optimized design by ourselves. Each dataset simply consists of CRPs. In our simulated dataset, the challenges are generated using the \textit{pypuf} \cite{pypuf} python library's random generator function as a set of $n$ length binary strings corresponding to the $n$ PUF length. Responses are generated by applying each challenge to each tested PUF instance, each of which is generated with a random seed (for each unique PUF). The seed is randomly chosen and guaranteed to differ for every simulated data generated in this article. 

\subsection{Attack Methodology}

A PUF can be considered `broken' if an adversary can successfully predict correct bits with a significant advantage above 50\% (the probability of correctly guessing the outcome of flipping a coin). Intuitively, as prediction accuracy is increased above 50\% per bit, the additional brute force work an adversary must carry out to determine the remaining bits of, say, an arbitrary length secret key is reduced. While there is no significant consensus\footnote{As of the publication of this work.} on a precise accuracy value to distinguish between a secure and vulnerable PUF, a threshold value of 70\% per-bit has been postulated in the literature. In the realm of cryptography, however, even advantages of  50\% +/- 2\% are thought to be insufficiently secure. Answering this question mathematically (with regard to key guessing), therefore, falls out of the scope of this work. However, we distinguish successful attacks for this work, whereby the difference between, say, 95\% prediction rate per-bit versus 99\% prediction rate both constitute a successful attack, given a 70\% threshold. We, therefore, do not aim at extremely high accuracy or the least amount of training CRPs on specific datasets but rather ensure the stability of the attack, given the complexity of the proposed attack (number/type of PUFs to be compromised). During the experiments, the strategy for every method is to begin the modelling at a reasonable amount of CRPs; then, if the attack succeeds with accuracy beyond $90\%$, we attempt more random PUFs. If an attempt fails, we increase the amount of CRP training data; otherwise, if the method models all the PUFs, we decrease the amount of training data and continue the test.

\subsection{Evaluations for Generic Framework of Single PUF}
% \todo[inline]{Maybe we need to prove first that it's reasonable to stop the accuracy competition after 95\%}
For our initial comparison, we present the experiment settings and results for the proposed generic framework of a single PUF. 


\subsubsection{Modelling Setup}
We implement our method and replicate other methods using Python 3.8 and TensorFlow 2.4 \cite{abadi2016tensorflow} back-end executed on a Windows laptop with 48 GB of main memory, 5GHz i9-12900H Intel(R) Core processor and NVIDIA GeForce RTX 3070 Ti Laptop GPU. The proposed method should to be generic for any composition of Arbiter-based PUFs; thus, we set up one model and experimented with this model with the same settings. In Section. \ref{sec:method}, we introduce the structure of the generic framework; here we show the hyperparameters used in experiments in Tab. \ref{tab:hp}. We use $Relu$ as the activation function for all the hidden layers, $Softmax$ for the gate function and $Sigmoid$ for the tower function. For all kinds of PUFs, the MoE has four experts, each with two fully connected hidden layers with $32$ neurons. We adjust the batch size according to the scale of the training dataset. Note the number of CRPs as $N_{crp}$, we set $batch\_size=min\{N_{crp},20000\}$. From the experiments, we find that dynamic adjustment can help the network to converge faster.
% As mentioned in Section. \ref{sec:exp}.
\begin{table}
    \centering
    \begin{threeparttable}
        \caption{Hyperparameter Value Used}
    \label{tab:hp}
    \begin{tabular}{cc}
        \toprule
        \textbf{Hyper Parameters} & \textbf{Values} \\
        \midrule
        Kernel Initializer & Glurot uniform \\
        Optimizer & Adam\cite{kingma2014adam} \\
        Hid. Lay. activ. & Relu \\
        Learning rate & Adaptive \\
        Loss function & BCE \\
        \bottomrule
    \end{tabular}
        \end{threeparttable}
\end{table}



\subsubsection{Modelling Accuracy Results on Simulated Dataset}
% We use \textit{pypuf}\footnote{\url{https://pypuf.readthedocs.io/}} \cite{pypuf} to generate simulated PUFs and datasets. The random seed is used to control the physical characteristics of PUFs. We randomly set the seed and tested each method with random PUFs. 

 As shown in Tab. \ref{tab:results_single}, we present the performance of our method on modelling XOR PUF and compare them with other state-of-the-art machine learning models.

% \textcolor{red}{Also some findings about the robustness of their methods. "Cursed PUF"}
Overall, our method successfully performs attacks on different structures of Arbiter-based PUFs without the need to change settings. With the benefit of a fixed structure, rather than a structure that expands as the PUF structure becomes more complex, the training time does not increase exponentially with the complexity of PUFs. From the accuracy results, we can find our method does not require more training CRPs to counteract the negative effects brought by the fixed network structure.


\begin{table}[ht]
    \centering
    \begin{threeparttable}
            \caption{modelling results of for Single XOR PUF on Simulated CRPs}
        \label{tab:results_single}
        \begin{tabular}{cccccc}
            \toprule
            % &  & \multicolumn{4}{c}{\textbf{Parameters}}\\
            \textbf{Method} & \textbf{k} & \textbf{crp} & \textbf{time} & \textbf{acc} & \textbf{Memory} \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling}& \multirow{3}{*}{2} & 8k & \textless20s & \textgreater 97.0\% &  1.78 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 8k & \textless20s & 97.0\% &  1.79 GiB \\ % &  
            \textbf{Mursi et al}\cite{Mursi}&  & 8k & \textless1m & \textgreater98\% &  1.86 GiB \\
            \textbf{Proposed Scheme}& & 8k & \textless 20s & $>$94\% & 2.06 GiB \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling}& \multirow{3}{*}{3} & 20k & \textless20s & \textgreater99.0\% &  1.84 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 24k & \textless20s & \textgreater97.0\% & 1.81 GiB \\ % &  
            \textbf{Mursi et al}\cite{Mursi}&  & 24k & \textless1m & \textgreater98\% &  1.88 GiB \\
            \textbf{Proposed Scheme}&  & 24k & \textless1m & $>$95\% & 2.15 GiB \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling}& \multirow{3}{*}{4} & 30k & \textless20s & \textgreater99.0\% &  1.91 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 100k & \textless1m & \textgreater98.0\% & 1.91 GiB \\ % &  
            \textbf{Mursi et al}\cite{Mursi}&  & 120k & \textless1m & \textgreater98.0\% &  1.97 GiB \\
            \textbf{Proposed Scheme}& & 80k & \textless1m & $>$97\% & 2.26 GiB \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling}& \multirow{3}{*}{5} & 260k & \textless20s & \textgreater99.0\% &  1.88 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 400k & \textless2m & \textgreater95.0\% &  2.32 GiB\\ % &  
            \textbf{Mursi et al}\cite{Mursi} &  & 240k & \textless1m & \textgreater98.0\% &  2.29 GiB \\
            \textbf{Proposed Scheme}& & 240k & \textless1m & 97.88\% & 2.24 GiB \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling}& \multirow{3}{*}{6} & 3M & \textless1m & \textgreater99.0\% &  2.34 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 1.6M & \textless2m & \textgreater99.0\% & 4.29 GiB \\ % &  
            \textbf{Mursi et al}\cite{Mursi}&  & 1.6M & \textless2m & \textgreater99.0\% &  3.04 GiB \\
            \textbf{Proposed Scheme}& & 800k & \textless10m & 95.56\% & 3.31 GiB \\
            \midrule
            \textbf{Rührmair et al}\cite{Ruhrmair_modelling} & \multirow{3}{*}{7} & 20M & \textless1h & \textgreater98\% &  4.61 GiB \\ % &  logistic regression
            \textbf{Aseeri et al}\cite{aseeri2018machine}&  & 5M &  \textless1h& \textgreater97\% & 8.05 GiB \\ % & 
            \textbf{Mursi et al}\cite{Mursi} & & 4M & \textless20m & \textgreater98.0\% & 8.07 GiB\\
            \textbf{Proposed Scheme}& & 2.4M & \textless10m & 98.61\% & 5.08 GiB \\
            \bottomrule
        \end{tabular}
        % &  \begin{tablenotes}
        % &      \small
        % &      \item[a] This is a footnote.
        % &      \item[b] This is another footnote.
        % &  \end{tablenotes}
    \end{threeparttable}
\end{table}

% \subsubsection{Comparison and Summary}
\paragraph{XOR Arbiter PUF}
We mainly refer to two state-of-the-art neural network models \cite{aseeri2018machine,Mursi} and one logistic regression model \cite{Ruhrmair_modelling} to compare our results. They offer detailed guidance for implementing the codes that can be easily replicated. Additionally, their claimed accuracy is close to our observations. To make the comparison fair and reasonable, we evaluate the performance of compared models by reproducing them using the same dataset and hardware resource. Besides our strategy for finding a stable amount of training data, we tried to find the best hyperparameters for compared schemes that were not claimed.

For the method presented by Rührmair et al. \cite{Ruhrmair_modelling}, we use code provided by Wisiol et al. in the PyPuf Python library \cite{pypuf}. This attack builds the network strictly according to the mathematical models. For small stages of XOR-APUFs, it outperforms all other methods in training time (lower is better) and accuracy. As stated in \cite{Nguyen_iPUF} \textbf{Theorem 1}, the logistic regression method is the most powerful attack among classical machine learning attacks; however, as the number of stages increases, LR consumes the most training data and time. Intuitively, when the number of XORs is more than 5, the deep learning method has more advantages. 
% we find the claimed attack on 5-XOR-APUF with 260k CRPs fails when the PUF seed is 5, the dataset seed is 2 and the model seed is 3. Thus we use 300k CRPs instead.

For the attacks presented by Asseri et al. in \cite{aseeri2018machine} and Mursi et al. in \cite{Mursi}, we implement their methods using the same setting claimed in their paper, including the kernel initializer, optimizer, learning rate, activation functions, and loss function. However, we optimize the batch size and adapt it according to the scale of training data. During the difficult reproducing work of different schemes, we find that the success of an attack highly relies on many factors: the dataset, the initial state of the model, the structure of the network, and even the batch size. Many ML-MA works indicate optimal accuracy and present their best accuracy on specific PUFs with few training CRPs. When we try to apply the method to a different dataset, it fails or can not achieve a reliable success rate. In some cases, different initialisations of the kernels succeed on different datasets and fail on others. The modelling process can be susceptible to differing hyperparameters. This kind of unreliable attack is unacceptable for realistic adversaries. Besides, methods Asseri et al. \cite{aseeri2018machine} and Mursi et al. \cite{Mursi} designed different structures for different PUFs. In most cases, they can not learn the PUFs of different types of PUFs, which means they need to know the type information. We discerned their acute sensitivity to the PUF's structure through our attack implementations on these schemes. This underscores the indispensability of type/structure information for mounting successful attacks. For instance, in \cite{Mursi}, the neural network devised for attacking a $k$-XOR Arbiter PUF comprises three fully connected hidden layers sized $\{2^{k-1},2^{k},2^{k}\}$. This implies that for a 5-XOR APUF and 6-XOR APUF, the hidden layer structures should be $\{2^{4},2^{5},2^{4}\}$ and $\{2^{5},2^{6},2^{5}\}$, respectively. We validated their efficacy on the stated CRP quantities, $200k$ and $200M$. Yet, when we experimented with the $\{2^{4},2^{5},2^{4}\}$-structure neural network for the 6-XOR APUF and the $\{2^{5},2^{6},2^{5}\}$-structure for the 5-XOR PUF, both attempts were unsuccessful. These outcomes underscore that non-generic models are meticulously crafted; simplistic models falter with complex PUFs, and conversely, intricate models struggle with simpler PUFs. Potential reasons could range from optimization challenges to under-fitting in the former scenario and over-fitting in the latter.

\textcolor{red}{Here we show why other models can not be ``generic model".}

\paragraph{XOR Feed-Forward Arbiter PUF and Interpose PUF}
In this section, we demonstrate the versatility of our model in adapting to a range of modelling tasks. Specifically, we apply our generic model to various more delay-based PUFs, encompassing even those PUFs previously resistant to successful attacks.

Avvaru et al. introduced the homogeneous and heterogeneous Feed-Forward XOR PUFs in \cite{avvaru2020homogeneous}. Subsequent to their work, a multitude of machine learning models were proposed to target FF-APUFs \cite{wisiol2022neural}. A large portion of these models capitalize on the inconsistent reliability of PUF designs, focusing particularly on homogeneous XOR FF PUFs with uniform loop positions. In contrast, heterogeneous XOR-FF-APUFs are largely considered resilient against modelling attacks. As evidenced in Figure. \ref{tab:results_FF_IPUF}, we successfully modeled $2-$loop FF PUFs with 2 XOR stages and $1-$loop FF PUFs with 3 XOR stages, achieving accuracy exceeding $95\%$ and $98\%$, respectively.

The Interpose PUF was introduced by Nguyen et al. in \cite{Nguyen_iPUF}. Although it was later targeted using the 'divide-and-conquer' technique \cite{Wisiol_split}, our results, as depicted in Figure. \ref{tab:results_FF_IPUF}, confirm that our proposed model can adeptly launch successful attacks on various configurations of the Interpose PUF without necessitating any structural alterations to the model itself.
\begin{table}
    \centering
    \begin{threeparttable}
            \caption{Modelling results of for Feed-Forward PUFs and Interpose PUFs}
        \label{tab:results_FF_IPUF}
        \begin{tabular}{p{1.5cm}ccccc}
            \toprule
            \textbf{Type} & \textbf{k} & \textbf{Loops} & \textbf{crp} & \textbf{time} & \textbf{acc} \\
            \midrule
             \multirow{12}{1.5cm}{\textbf{Homogeneous FF-PUF}} & \multirow{5}{*}{1} & 1 & 20k & $<$2m & $>$94\% \\
             &  & 2 & 120k & $<$2m & $>$97\% \\
             &  & 3 & 250k & $<$2m & $>$98\% \\
             &  & 4 & 500k & $<$2m & $>$98\% \\
             &  & 5 & 1M & $<$10m & $>$94\% \\
             \cmidrule(lr){3-6}
             & \multirow{5}{*}{2} & 1 & 90k & $<$2m & $>$93\% \\
             &  & 2 & 200k & $<$10m & $>$97\% \\
             &  & 3 & 400k & $<$10m & $>$93\% \\
             &  & 4 & 800k & $<$20m & $>$85\% \\
             &  & 5 & 1.6M & $<$1h & $>$90\% \\
             \cmidrule(lr){3-6}
             & \multirow{2}{*}{3} & 1 & 120k & $<$2m & $>$90\% \\
             &  & 2 & 400k & $<$10m & $>$93\% \\
            %  & 3 & 3 20k & $<$2m & $>$94\% \\
            \midrule
            \multirow{3}{1.5cm}{\textbf{Heterogeneous FF-PUF}} & 2 & 1 & 160k & $<$2m & $>$98\% \\
            & 3 & 1 & 640k & $<$10m & $>$98\% \\
            & 2 & 2 & 320k & $<$2m & $>$95\%\\
            \midrule
            \multirow{4}{1.5cm}{\textbf{Interpose PUF}} & \textbf{Upper chains} & \textbf{Lower chains} & \textbf{crp} & \textbf{time} & \textbf{acc} \\
            & 1 & 5 & 480k & $<$2m & $>$98\% \\
            & 3 & 3 & 320k & $<$3m & $>$98\% \\
            & 4 & 4 & 800k & $<$1h & $>$96\% \\
            & 5 & 5 & 2M & $<$1h & $>$96\% \\
            \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table}



\subsubsection{Modelling Accuracy Results on Silicon CRPs}
To avoid faulty evaluations caused by wrongly generated simulated data, we validate our method on real-world data provided by Mursi et al.\cite{Mursi}. We randomly select the demand amount of CRPs from the silicon data and apply our framework without changing any model settings, which is needed for all other models. The results are shown in Figure. \ref{tab:results_single_real}. we can find the accuracy does not decrease at all for any stage of XOR-APUFs when we use the same amount of CRPs.

\begin{table}
    \centering
    \begin{threeparttable}
            \caption{Modelling results of for Single XOR PUF on Silicon CRPs.}
        \label{tab:results_single_real}
        \begin{tabular}{ccccccc}
            \toprule
            & \multicolumn{3}{c}{\textbf{Mursi et al.\cite{Mursi}}} & \multicolumn{3}{c}{\textbf{Our data}} \\
            \cmidrule(lr){2-4} \cmidrule(lr){5-7}
            \textbf{k} & \textbf{crp} & \textbf{time} & \textbf{acc} & \textbf{crp} & \textbf{time} & \textbf{acc} \\
            \midrule
            % 2 & - & - & -& 8k & \textless20s & 92.80\% \\
            % 3 & - & - & -& 20k & \textless20s & 90.70\% \\
            4 & 40k & \textless20s & 92.56\% & 40k & \textless20s & 92.90\% \\
            % \midrule
            5 & 160k & \textless20s & 95.21\%& 120k & \textless1m & 95.36\% \\
            % \midrule
            6 & 560K & \textless1m & 94.56\% & 120k & \textless1m & 95.36\%\\
            % \midrule
            7 & 1.6M & \textless1m & 93.38\% & 600k & \textless10m & 95.81\%\\
            \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table}

Then we implement 64-stages Arbiter PUFs on our Zynq-7000 FPGA using Vivado design suite. Verilog hardware description language to build the PUF design. No placement design is applied to these PUFs. The hardware layout is shown in Figure. \ref{fig:hardware}. We applied DRAM controller to transfer challenges and obtain responses between the PL and PS sides. For each single Arbiter PUF, we evaluate its performance.

\begin{figure}[ht]
\begin{center}
\makebox[0pt]{\includegraphics[width=78mm]{imgs/7PUFs.png}}
\end{center}
\caption{Hardware layout for $7$ PUFs on XC7Z010 FPGA Board. No optimization design for the layout was performed.}
\label{fig:hardware}
\end{figure}

\todo[inline]{Where to put this paragraph}
\subsubsection{Resource Consumption and Efficiency Analysis}
In many modeling attack work targeting on PUFs \cite{wisiol2022neural, Santikellur_composition, Mursi,aseeri2018machine}, the structure of models varies for different PUFs. For our framework being designed for a generic purpose, it is not suitable to compare the scale of models directly for consumption evaluations. However, we list the time cost and memory usage in Fig. \ref{tab:results_single}. The time cost of our proposed scheme makes not much difference from other compared methods and outperforms Rührmair et al \cite{Ruhrmair_modelling} and Aseeri et al \cite{aseeri2018machine} when attacking 7-XOR APUF. We used more memory in our scheme for attacking that more neurons and layers are used in our model. For 7-XOR APUF, 5.08 GiB memory is needed, as methods in \cite{Ruhrmair_modelling, aseeri2018machine, Mursi}, 4.61, 8.05, 8.07 GiB is needed. We clarify here that our memory usage might be different as they were claimed, in addition to the hardware differences, we used larger batch sizes to speed up the training. For our model, the memory usage between different tasks mainly depends on the amount of dataset, which determines the batch size. Overall, we fixed the structure for all types of PUFs and the most complex PUF determines the hardware requirement for our model.


\subsection{Evaluations for Generic Framework of Multiple PUFs}
In the above, we have shown the generality of the proposed model that we do not need to design specific structures for different types of PUFs and no information apart from CRPs is needed. Then we evaluate another generic property of our proposed model on multiple tasks. To the best of our knowledge, multiple-task learning for multiple PUFs has not been studied before. In this section, we first show how multiple tasks learning challenges the existing modeling methods and compare them with ours. Then we present our modelling accuracy results on different combinations of different types of PUFs.

\subsubsection{Comparison and Summary}
We managed to employ extra output layers on contrasting schemes listed above to enable their multi-task learning capability. After the modifications, their models look like the share-bottoms \cite{caruana1997multitask}.

For \cite{Ruhrmair_modelling}, we cannot add output layers for a mathematical-model-based structure since they used multiplying layers and output the result after the activation function directly. 

For \cite{Mursi,aseeri2018machine}, we add one extra output layer. The results for modelling multiple XOR PUFs are shown in Tab. \ref{tab:results_multiple_comb}. The results show that their models can not balance between different tasks and will always fail one random task, which is described as the result of "Negative Transfer" when the two tasks have low similarity or the experts cannot understand the correlation. In this case, multiple-task learning does not work and even the performance for training the single task is also degraded by the other conflicting task. However, as shown in Tab. \ref{tab:results_multiple_comb}, our proposed model can deal with different tasks with good performance, compared to the same single task.

We also list more combinations of different numbers of different PUFs in Tab. \ref{tab:combinations} to show the flexibility of the proposed model. In comb. \uppercase\expandafter{\romannumeral 1}, we show the results of modeling four XOR APUFs with the same stages and different stages. In comb. \uppercase\expandafter{\romannumeral 2}, we show the results of modeling four XOR FF-APUFs with different types. In comb. \uppercase\expandafter{\romannumeral 3}, we show the results for different combinations of XOR APUFs, XOR FF-APUFs, and Interpose PUFs. Compared to the results in Tab. \ref{tab:results_single}, $3\%$ of accuracy is traded off in average and the maximum is around $8\%$.

\subsubsection{Modelling Accuracy Results}
We present a variety of combinations using different quantities and types of PUFs in Tab. \ref{tab:combinations} to demonstrate the versatility of our proposed model. In combination \uppercase\expandafter{\romannumeral 1}, we showcase results from modeling four XOR APUFs, both with consistent and varying stages. In combination \uppercase\expandafter{\romannumeral 2}, we illustrate the outcomes when modeling four distinct types of XOR FF-APUFs. For combination \uppercase\expandafter{\romannumeral 3}, we exhibit results derived from a mixture of XOR APUFs, XOR FF-APUFs, and Interpose PUFs. When juxtaposed with the outcomes in Tab. \ref{tab:results_single}, there's an average accuracy reduction of $3\%$, with the maximum drop close to $8\%$

\begin{table}[ht]
    \centering
    \begin{threeparttable}
            \caption{Modelling results of for Multiple(\textbf{Two}) XOR PUFs on Simulated CRPs}
        \label{tab:results_multiple_comb}
        \begin{tabular}{ccccc}
            \toprule
            % & \multicolumn{4}{c}{\textbf{Parameters}}\\
            \textbf{Method} & \textbf{k} & \textbf{crp} & \textbf{time} & \textbf{acc} \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{2} & 10k & \textless20s & 71.5\% \\ % 
            \textbf{Mursi et al}\cite{Mursi}&  & 10k & \textless20s & 67.34\% \\
            \textbf{Proposed Scheme}& & 8k & \textless 20s & 93.50\% \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{3} & 30k & \textless20s & 72\% \\ % 
            \textbf{Mursi et al}\cite{Mursi}&  & 30k & \textless20s & 74.39\% \\
            \textbf{Proposed Scheme}&  & 24k & \textless20s & 93.02\% \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{4} & 100k & \textless20s & 73.72\% \\ % 
            \textbf{Mursi et al}\cite{Mursi}&  & 100k & \textless20s & 74.60\% \\
            \textbf{Proposed Scheme}& & 40k & \textless20s & 93.99\% \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{5} & 400k & \textless20s & 50\% \\ % 
            \textbf{Mursi et al}\cite{Mursi} &  & 400k & \textless20s & 74.89\% \\
            \textbf{Proposed Scheme}& & 240k & \textless20s & 97.88\% \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{6} & 2M & \textless1m & 74.08\% \\ % 
            \textbf{Mursi et al}\cite{Mursi}&  & 2M & \textless1m & 74.08\% \\
            \textbf{Proposed Scheme}& & 800k & \textless20s & 95.04\% \\
            \midrule
            \textbf{Aseeri et al}\cite{aseeri2018machine}& \multirow{3}{*}{7} & 5M & \textless5m & 74.20\% \\ %
            \textbf{Mursi et al}\cite{Mursi} & & 5M & \textless5m & 50\% \\
            \textbf{Proposed Scheme}& & 1.6M & \textless2m & 98.04\% \\
            \bottomrule
        \end{tabular}
        % \begin{tablenotes}
        %     \small
        %     \item[a] This is a footnote.
        %     \item[b] This is another footnote.
        % \end{tablenotes}
    \end{threeparttable}
\end{table}

In Tab. \ref{tab:combinations}, we show the attacking results of our proposed model on different combinations of delay-based PUFs.

\begin{table*}[ht]
\scriptsize
\begin{threeparttable}
\setlength\tabcolsep{5pt} % Adjust column separation here
\centering
\caption{Results of Attacking Different Combinations of Different PUFs with Our Proposed Scheme}
\label{tab:combinations}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} ccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Comb. No.}}&\multicolumn{3}{c}{\textbf{XOR APUF}\tnote{\textdagger}} & \multicolumn{3}{c}{\textbf{XOR FF-APUF}\tnote{\textdagger\textdagger}} & \multicolumn{3}{c}{\textbf{Interpose PUF}\tnote{\textdaggerdbl}}& \textbf{Numbers } & \multicolumn{2}{c}{\textbf{Performance}} \\
\cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-10} \cmidrule{12-13}
 &\textbf{3} & \textbf{4} & \textbf{5} & \textbf{2-1} & \textbf{2-2} & \textbf{1-3} & \textbf{(1, 5)} & \textbf{(2, 2)} & \textbf{(3, 3)} & \textbf{of PUFs} & \textbf{Average Accuracy} & \textbf{Running time} \\
\midrule
% - & - & - & - & - & - & - & - & - & $>$93\%& $<$1m  \\
\multirow{4}{*}{\uppercase\expandafter{\romannumeral 1}}&4 & - & - & - & - & - & - & - & - & 4 &$>$93\%& $<$2m  \\
                                       &- & 4 & - & - & - & - & - & - & - & 4 &$>$93\%& $<$10m  \\
                                       &- & - & 4 & - & - & - & - & - & - & 4 &$>$94\%& $<$20m  \\
                                       &2 & 2 & 1 & - & - & - & - & - & - & 5 &$>$92\%& $<$10m  \\
\cmidrule{2-13}
\multirow{2}{*}{\uppercase\expandafter{\romannumeral 2}}&- & - & - & 4 & - & - & - & - & - & 4 &$>$95\%& $<$20m  \\
                                       &- & - & - & - & - & 4 & - & - & - & 4 &$>$92\%& $<$30m  \\
\cmidrule{2-13}
\multirow{4}{*}{\uppercase\expandafter{\romannumeral 3}}&- & - & - & - & - & - & 4 & - & - & 4 &$>$96\%& $<$30m  \\
                                       &2 & 2 & - & - & - & - & 1 & - & - & 5 &$>$96\%& $<$30m  \\
                                       &- & - & - & 1 & 1 & 1 & 1 & - & - & 4 &$>$90\%& $<$30m  \\
                                       &- & - & - & - & - & - & 1 & 1 & 1 & 3 &$>$90\%& $<$30m  \\

\bottomrule
\end{tabular*}
\smallskip
\scriptsize
\begin{tablenotes}
\item[\textdagger] The parameter indicate the number of XOR stages;
\item[\textdagger\textdagger] The two parameters indicate the number of XOR stages and loops;
\item[\textdaggerdbl] The parameter indicate the number of parallel arbiter chains in up and lower layers.
\item[*] In the table, the amount of training data for each PUF is the same with corresponding single task.
\end{tablenotes}
\end{threeparttable}
\end{table*}



% \begin{table}
%     \centering
%     \begin{threeparttable}
%             \caption{modelling results for Multiple XOR PUFs}
%         \label{tab:results_multiple_comb}
%         \begin{tabular}{ccccc}
%             \toprule
%             Combination & crp & time & avg acc \\
%             \midrule
%              $2\times$ 2-XOR & 10k & \textless20s & \textgreater93\% \\
%             % \midrule
%              $2\times$ 3-XOR & 30k & \textless20s & \textgreater93\% \\
%             % \midrule
%             $2\times$ 4-XOR & 60k & \textless20s & \textgreater93\% \\
%             % \midrule
%             $2\times$ 5-XOR & 200k & \textless20s & \textgreater93\% \\
%             % \midrule
%             $2\times$ 6-XOR & 800k & \textless1m & \textgreater93\% \\
%             % \midrule
%             $2\times$ 7-XOR & 2M & \textless5m & \textgreater93\% \\
%             \bottomrule
%         \end{tabular}
%         % \begin{tablenotes}
%         %     \small
%         %     \item[a] This is a footnote.
%         %     \item[b] This is another footnote.
%         % \end{tablenotes}
%     \end{threeparttable}
% \end{table}

% \begin{table}[t]
%     \centering
%     \begin{threeparttable}
%             \caption{modelling results of \cite{aseeri2018machine} for Multiple XOR PUFs}
%         \label{tab:results_mul_asee}
%         \begin{tabular}{ccccc}
%             \toprule
%             Combination & crp & time & avg acc \\
%             \midrule
%              $2\times$ 2-XOR & 10k & \textless20s & 71.5\% \\
%             % \midrule
%              $2\times$ 3-XOR & 30k & \textless20s & 72\% \\
%             % \midrule
%             $2\times$ 4-XOR & 100k & \textless20s & 73.72\% \\
%             % \midrule
%             $2\times$ 5-XOR & 400k & \textless20s & 50\% \\
%             % \midrule
%             $2\times$ 6-XOR & 2M & \textless1m & 74.08\% \\
%             % \midrule
%             $2\times$ 7-XOR & 5M & \textless5m & 74.20\% \\
%             \bottomrule
%         \end{tabular}
%         % \begin{tablenotes}
%         %     \small
%         %     \item[a] This is a footnote.
%         %     \item[b] This is another footnote.
%         % \end{tablenotes}
%     \end{threeparttable}
% \end{table}
% \begin{table}[t]
%     \centering
%     \begin{threeparttable}
%             \caption{modelling results of \cite{Mursi} for Multiple XOR PUFs}
%         \label{tab:results_mul_mur}
%         \begin{tabular}{ccccc}
%             \toprule
%             Combination & crp & time & avg acc \\
%             \midrule
%              $2\times$ 2-XOR & 10k & \textless20s & 67.34\% \\
%             % \midrule
%              $2\times$ 3-XOR & 30k & \textless20s & 74.39\% \\
%             % \midrule
%             $2\times$ 4-XOR & 100k & \textless20s & 74.60\% \\
%             % \midrule
%             $2\times$ 5-XOR & 400k & \textless20s & 74.89\% \\
%             % \midrule
%             $2\times$ 6-XOR & 2M & \textless1m & 74.08\% \\
%             % \midrule
%             $2\times$ 7-XOR & 5M & \textless5m & 50\% \\
%             \bottomrule
%         \end{tabular}
%         % \begin{tablenotes}
%         %     \small
%         %     \item[a] This is a footnote.
%         %     \item[b] This is another footnote.
%         % \end{tablenotes}
%     \end{threeparttable}
% \end{table}

==> sections/Methodology.tex <==
\section{Proposed Generic Framework}
\label{sec:method}
% \subsection{Motivation}
As discussed in Section \ref{sec:related}, numerous modelling attack methods \cite{RN174,Mursi,RN38,santikellur2019computationally} have demonstrated commendable prediction accuracy in PUF responses. A shared characteristic among these methods is their reliance on the type or structure of the target PUF as foundational information for modelling. Typically, traditional machine-learning-based models are intricately tailored for a specific PUF type, exhibiting prowess in predicting unacquired CRPs with remarkable precision. Beyond the issue of generality, as delineated in the adversary model \ref{sub:model}, acquiring such information covertly within a network is impractical. Expecting an adversary to test every possible structure while targeting a PUF is also illogical, given the varying amounts of training data required for different PUFs to orchestrate a successful assault. We introduce a generic framework to address these challenges of generality and type information absence in PUF modelling. Here, a singular neural network structure is employed to model diverse PUF types, irrespective of prior type knowledge. An extended version is also proposed to perform multiple-PUF modelling on the combinations of several of the same or different PUFs. As discussed in Section. \ref{sec:related}, many types of delay-based-Strong PUFs share structural similarities. Therefore, it is intuitive to to utilise this structural similarity and capture the relationship across these differing PUF instances during modelling when preparing a ML-MA.

\subsection{Generic Framework for a Single PUF}
\label{sub:generic_single}
% \todo[inline]{Similarity(Motivation)}

\begin{figure}[t!]
\begin{center}
\makebox[0pt]{\includegraphics[width=\linewidth]{imgs/MoE_1PUF.pdf}}
\end{center}
\caption{Generic Framework of a Single PUF.}
\label{fig:moe_1puf}
\end{figure}

We incorporate the MoE structure \cite{MMoE}, as briefly outlined in Section \ref{subsec:MMoE}. The structure is depicted in Figure. \ref{fig:moe_1puf}, the model accepts a challenge as input and produces the predicted response as output. Challenges are processed by an input layer connected to three experts. These experts are tailored to handle the distinct features of CRPs. Each expert comprises two hidden layers, each with $32$ neurons. The first layer is directly connected to the input layer, while the second links to the gate function. The gate function assigns weights to the experts, amalgamates their outputs, and channels them to the tower. 
Initially, we convert the challenge bits $C^{N}$ (where $N$ represents the PUF stages) into the feature vector $X^{N}$, aligning with the structure of the arbiter-based PUF \textcolor{red}{(a reference to the additive delay model is required)}:
\begin{equation}
x_{i}=\prod_{j=i}^{n}c_{j}
\end{equation}
This transformation aids the model in perceiving the decision boundary as a hyperplane. The response $r$ serves as the labels and is adjusted to the range ${0,1}$, if not already within it, to align with the activation function.
Post-feature engineering, the input layer is structured to accommodate these features. In the MOE layer, we establish $K$ experts, with the count being adaptable based on species quantity. The expert structure remains consistent across all PUF types, as two hidden layers equipped with non-linear activation functions are believed to model any function, given sufficient parameters. The $k-$th expert, denoted as $f_{k}(\cdot)$, is designed to extract specific insights or features from the input. Each expert delivers their unique interpretation of the input: $h_{k}(X)=f_{k}(X^{n})$.

To harness the expertise of various experts without overburdening the model with excessive parameters, we introduce the gate function $g(x)$. This function evaluates the features and determines the weight. We employ the $softmax(\cdot)$ activation function post the $N\times K$ kernel $W_{gk}$ to distribute weights among experts and ensure the model prioritises the most apt one. Consequently, weights are computed as: $g(X)=softmax(W_{NK}(X))$. The weight assigned to the $k$-th expert is represented as $g^{k}(X)$, ensuring that $\sum_{k=1}^{K}g^{k}(X)=1$. Subsequently, the MOE layer's output is derived by amalgamating the outputs of the experts: $moe(X)=\sum_{i=1}^{K}g^{i}(X)h_{i}(X)$. We then establish the tower layer, $T(\cdot)$, tasked with processing the composite information supplied by the experts. This layer then connects to the output layer, which employs the $sigmoid(\cdot)$ activation function to restrict the prediction output to the range ${0,1}$. Our rationale for selecting a dual-layer hidden structure aligns with the perspective of Wisiol et al. in \cite{wisiol2022neural}. Viewing neural networks as a potent instrument for PUF modelling, we are confident that, given ample parameters and layers, PUFs can be effectively modelled, barring optimization constraints. Fewer layers expedite model convergence. Additionally, the MOE structure's inherent flexibility allows the gate function to integrate multiple experts, facilitating network scalability to accommodate the diverse complexities inherent to PUFs.


% \textcolor{red}{We will explore several state-of-the-art and classic schemes in Section \ref{sec:exp}} 
% \todo[inline]{Need to ensure consistent use of terminology WRT classical, traditional ML methods throughout paper - we discuss these in related works and ML-MA background section}.

% (The activation function for all the hidden layers are 'relu', for the output layer is 'sigmoid'.)


\subsection{Generic Framework for Multiple PUFs}
\label{subsec:method_mul}
This section extends the framework to a multiple-task learning model to enable the attack over multiple unique PUF instances. As discussed in Section \ref{sub:PUF}, the additive delay function represents the inner interaction of PUFs. We can find that they share similar mathematical formulations for the same category of PUF. Taking XOR-Arbiter-PUF as an example, for a $k$-XOR APUF, the responses can be represented as $f(c)=\operatorname{sgn}( \prod_{l=1}^k\left(\left\langle W_l, x\right\rangle+b_l\right))$, signifying that various modelling tasks exhibit commonalities as they employ an identical mathematical representation with varying parameter (delay) values. Thus, a multiple-tasks framework can help improve the modelling performance. The structure of the generic framework for multiple PUFs is shown in Fig. \ref{fig:moe_mpuf}. 

The number of experts can be customized according to the potential types and numbers of PUFs. The idea is that different structures or numbers of neurons in hidden layers are suitable for different types of PUF. For some simple PUFs, if the model is too complex, it will be hard for the model to converge without a large amount of training data. This can also be concluded from the comparison results shown by Wisiol et al in \cite{wisiol2022neural}. In this case, the gate function helps choose the suitable expert from the MoE layer can alleviate optimization problems caused by too large a model. In Section \ref{subsec:MMoE}, we have already shown how to build the multiple-PUFs model based on MMoE. As shown in Fig. \ref{fig:moe_mpuf}, we give an example of modelling two PUFs simultaneously. As mentioned in Section. \ref{sub:generic_single}, the feature engineering and input layer remain the same. The expert structure is also the same, but the number of experts may differ according to the number of PUFs.

There are $N_{PUFs}$ gate functions, tower functions and output layers for $N_{PUFs}$ PUF models, so-called as $N_{PUFs}$ tasks. For the $t$-th task, the weighed output of MOE layer is:
\begin{equation}
    moe^{t}(X)=\sum_{i=1}^{K}g^{i}_{t}(X)h_{i}(X)
\end{equation}
Then, the specific tower $T_{t}(\cdot)$ for task $t$ will deal with the extracted features provided by the experts and forward the results to the output layer to give the prediction.

\begin{figure}[t!]
\begin{center}
\makebox[0pt]{\includegraphics[width=78mm]{imgs/MoE_MPUF.pdf}}
\end{center}
\caption{Generic Framework of Multiple PUFs.}
\label{fig:moe_mpuf}
\end{figure}


% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{imgs/MoE_1PUF.png}
%         \caption{Generic Framework of Single PUF.}
%         \label{fig:moe_1puf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{imgs/MoE_MPUF.png}
%         \caption{Generic Framework of Multiple PUFs.}
%         \label{fig:moe_mpuf}
%     \end{subfigure}
%     \caption{Combined Figure with Subfigures}
%     \label{fig:combined_figure}
% \end{figure}


% \subsection{Feature Engineering}

% \subsection{Compositions in Arbiter-based PUF}


==> sections/Overall_meth.tex <==
\section{Proposed Generic Framework}
\label{sec:method}
% \subsection{Motivation}
As discussed in Section \ref{sec:related}, numerous modelling attack methods \cite{RN174,Mursi,RN38,santikellur2019computationally} have demonstrated commendable prediction accuracy in PUF responses. A shared characteristic among these methods is their reliance on the type or structure of the target PUF as foundational information for modelling. Typically, traditional machine-learning-based models are intricately tailored for a specific PUF type, exhibiting prowess in predicting unacquired CRPs with remarkable precision. Beyond the issue of generality, as delineated in the adversary model \ref{sub:model}, acquiring such information covertly within a network is impractical. Expecting an adversary to test every possible structure while targeting a PUF is also illogical, given the varying amounts of training data required for different PUFs to orchestrate a successful assault. We introduce a generic framework to address these challenges of generality and type information absence in PUF modelling. Here, a singular neural network structure is employed to model diverse PUF types, irrespective of prior type knowledge. An extended version is also proposed to perform multiple-PUF modelling on the combinations of several of the same or different PUFs. As discussed in Section. \ref{sec:related}, many types of delay-based-Strong PUFs share structural similarities. Therefore, it is intuitive to to utilise this structural similarity and capture the relationship across these differing PUF instances during modelling when preparing a ML-MA.

\subsection{Generic Framework for a Single PUF}
\label{sub:generic_single}
% \todo[inline]{Similarity(Motivation)}

\begin{figure}[t!]
\begin{center}
\makebox[0pt]{\includegraphics[width=78mm]{imgs/MoE_1PUF.png}}
\end{center}
\caption{Generic Framework of a Single PUF.}
\label{fig:moe_1puf}
\end{figure}

We incorporate the MoE structure \cite{MMoE}, as briefly outlined in Section \ref{subsec:MMoE}. The structure is depicted in Figure \ref{fig:moe_1puf}, the model accepts a challenge as input and produces the predicted response as output. Challenges are processed by an input layer connected to three experts. These experts are tailored to handle the distinct features of CRPs. Each expert comprises two hidden layers, each with $32$ neurons. The first layer is directly connected to the input layer, while the second links to the gate function. The gate function assigns weights to the experts, amalgamates their outputs, and channels them to the tower. 
Initially, we convert the challenge bits $C^{N}$ (where $N$ represents the PUF stages) into the feature vector $X^{N}$, aligning with the structure of the arbiter-based PUF \textcolor{red}{(a reference to the additive delay model is required)}:
\begin{equation}
x_{i}=\prod_{j=i}^{n}c_{j}
\end{equation}
This transformation aids the model in perceiving the decision boundary as a hyperplane. The response $r$ serves as the labels and is adjusted to the range ${0,1}$, if not already within it, to align with the activation function.
Post-feature engineering, the input layer is structured to accommodate these features. In the MOE layer, we establish $K$ experts, with the count being adaptable based on species quantity. The expert structure remains consistent across all PUF types, as two hidden layers equipped with non-linear activation functions are believed to model any function, given sufficient parameters. The $k-$th expert, denoted as $f_{k}(\cdot)$, is designed to extract specific insights or features from the input. Each expert delivers their unique interpretation of the input: $h_{k}(X)=f_{k}(X^{n})$.

To harness the expertise of various experts without overburdening the model with excessive parameters, we introduce the gate function $g(x)$. This function evaluates the features and determines the weight. We employ the $softmax(\cdot)$ activation function post the $N\times K$ kernel $W_{gk}$ to distribute weights among experts and ensure the model prioritises the most apt one. Consequently, weights are computed as: $g(X)=softmax(W_{NK}(X))$. The weight assigned to the $k$-th expert is represented as $g^{k}(X)$, ensuring that $\sum_{k=1}^{K}g^{k}(X)=1$. Subsequently, the MOE layer's output is derived by amalgamating the outputs of the experts: $moe(X)=\sum_{i=1}^{K}g^{i}(X)h_{i}(X)$. We then establish the tower layer, $T(\cdot)$, tasked with processing the composite information supplied by the experts. This layer then connects to the output layer, which employs the $sigmoid(\cdot)$ activation function to restrict the prediction output to the range ${0,1}$. Our rationale for selecting a dual-layer hidden structure aligns with the perspective of Wisiol et al. in \cite{wisiol2022neural}. Viewing neural networks as a potent instrument for PUF modelling, we are confident that, given ample parameters and layers, PUFs can be effectively modelled, barring optimization constraints. Fewer layers expedite model convergence. Additionally, the MOE structure's inherent flexibility allows the gate function to integrate multiple experts, facilitating network scalability to accommodate the diverse complexities inherent to PUFs.


% \textcolor{red}{We will explore several state-of-the-art and classic schemes in Section \ref{sec:exp}} 
% \todo[inline]{Need to ensure consistent use of terminology WRT classical, traditional ML methods throughout paper - we discuss these in related works and ML-MA background section}.

% (The activation function for all the hidden layers are 'relu', for the output layer is 'sigmoid'.)


\subsection{Generic Framework for Multiple PUFs}
\label{subsec:method_mul}
This section extends the framework to a multiple-task learning model to enable the attack over multiple unique PUF instances. As discussed in Section \ref{sub:PUF}, the additive delay function represents the inner interaction of PUFs. We can find that they share similar mathematical formulations for the same category of PUF. Taking XOR-Arbiter-PUF as an example, for a $k$-XOR APUF, the responses can be represented as $f(c)=\operatorname{sgn}( \prod_{l=1}^k\left(\left\langle W_l, x\right\rangle+b_l\right))$, signifying that various modelling tasks exhibit commonalities as they employ an identical mathematical representation with varying parameter (delay) values. Thus, a multiple-tasks framework can help improve the modelling performance. The structure of the generic framework for multiple PUFs is shown in Fig. \ref{fig:moe_mpuf}. 

The number of experts can be customized according to the potential types and numbers of PUFs. The idea is that different structures or numbers of neurons in hidden layers are suitable for different types of PUF. For some simple PUFs, if the model is too complex, it will be hard for the model to converge without a large amount of training data. This can also be concluded from the comparison results shown by Wisiol et al in \cite{wisiol2022neural}. In this case, the gate function helps choose the suitable expert from the MoE layer can alleviate optimization problems caused by too large a model. In Section \ref{subsec:MMoE}, we have already shown how to build the multiple-PUFs model based on MMoE. As shown in Fig. \ref{fig:moe_mpuf}, we give an example of modelling two PUFs simultaneously. As mentioned in Section. \ref{sub:generic_single}, the feature engineering and input layer remain the same. The expert structure is also the same, but the number of experts may differ according to the number of PUFs.

There are $N_{PUFs}$ gate functions, tower functions and output layers for $N_{PUFs}$ PUF models, so-called as $N_{PUFs}$ tasks. For the $t$-th task, the weighed output of MOE layer is:
\begin{equation}
    moe^{t}(X)=\sum_{i=1}^{K}g^{i}_{t}(X)h_{i}(X)
\end{equation}
Then, the specific tower $T_{t}(\cdot)$ for task $t$ will deal with the extracted features provided by the experts and forward the results to the output layer to give the prediction.

\begin{figure}[t!]
\begin{center}
\makebox[0pt]{\includegraphics[width=78mm]{imgs/MoE_MPUF.png}}
\end{center}
\caption{Generic Framework of Multiple PUFs.}
\label{fig:moe_mpuf}
\end{figure}


% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{imgs/MoE_1PUF.png}
%         \caption{Generic Framework of Single PUF.}
%         \label{fig:moe_1puf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{imgs/MoE_MPUF.png}
%         \caption{Generic Framework of Multiple PUFs.}
%         \label{fig:moe_mpuf}
%     \end{subfigure}
%     \caption{Combined Figure with Subfigures}
%     \label{fig:combined_figure}
% \end{figure}


% \subsection{Feature Engineering}

% \subsection{Compositions in Arbiter-based PUF}

